Received Power Maximization Using Nonuniform Discrete Phase Shifts for RISs With a Limited Phase Range

To maximize the received power at a user equipment, the problem of optimizing a reconfigurable intelligent surface (RIS) with a limited phase range R < 2{\pi} and nonuniform discrete phase shifts with adjustable gains is addressed. Necessary and sufficient conditions to achieve this maximization are given. These conditions are employed in two algorithms to achieve the global optimum in linear time for R {\ge} {\pi} and R < {\pi}, where R is the limited RIS phase range. With a total number of N(2K + 1) complex vector additions, it is shown for R {\ge} {\pi} and R < {\pi} that the global optimality is achieved in NK or fewer and N(K + 1) or fewer steps, respectively, where N is the number of RIS elements and K is the number of discrete phase shifts which may be placed nonuniformly over the limited phase range R. In addition, we define two quantization algorithms that we call nonuniform polar quantization (NPQ) algorithm and extended nonuniform polar quantization (ENPQ) algorithm, where the latter is a novel quantization algorithm for RISs with a significant phase range restriction, i.e., R < {\pi}. With NPQ, we provide a closed-form solution for the approximation ratio with which an arbitrary set of nonuniform discrete phase shifts can approximate the continuous solution. We also show that with a phase range limitation, equal separation among the nonuniform discrete phase shifts maximizes the normalized performance. Furthermore, we show that the gain of using K {\ge} 3 with R < {\pi}/2 and K {\ge} 4 with R < {\pi} is only marginal. Finally, we prove that when R < 2{\pi}/3, ON/OFF selection for the RIS elements brings significant performance compared to the case when the RIS elements are strictly ON.

==> Introduction0.tex <==
%
\section{Introduction}\label{ch:0}
%
%Reference \cite{b1} presented an algorithm to solve
In wireless communications, the performance demand has significantly grown with the advancements in technology, requiring to cope with many challenges in the propagation environment. In dense urban outdoor-indoor areas, the problems of shadowing and fading can become severe. In specific scenarios where the direct link between the base stations and users is blocked, despite the more extensive beamforming capability of the base stations, the performance can be significantly degraded \cite{ABCHLSZ14}. In order to catch up with the ever-growing quality of service (QoS) and energy efficiency requirements in mobile communications, the challenges due to blockages must be overcome to prevent performance degradation \cite{BDDDAZ19}.

A reconfigurable intelligent surface (RIS), also known as intelligent reflective surface (IRS), can manipulate the incident electromagnetic waves to control the propagation environment by varying the phases of the incident signals with its low-cost passive reflecting elements \cite{ACS22}. In recent years, RISs have been studied in many communication systems in the literature, and it is shown that RIS can become a crucial enabler for communication environments, especially when there is a loss in line-of-sight (LOS) between the base station (BS) and user equipment (UE) \cite{BWMPSC22},\cite{PYTCLWZB21}. 

For complex communication scenarios, algorithms are developed with the assumption of continuous phase shifts at the RIS, for ease of optimization \cite{YXS20},\cite{YXS19},\cite{WZ19}. In \cite{YXS20}, to achieve a globally optimal solution, the authors developed an algorithm which is based on the branch-and-bound method. In \cite{YXS19}, the authors developed a secure wireless communication system for a single-user case by adopting the majorization-minimization and block coordinate descent (BCD) techniques. Assuming perfect knowledge of the channels in \cite{WZ19}, the authors jointly designed the active and passive beamforming to minimize the transmit power, subject to individual signal-to-interference-ratio constraints of the users. A two-tier approach is employed to deal with discrete constraints in \cite{WGWM23}, where the authors minimized the required transmit power at the BS, with a proposed penalty-based algorithm and manifold optimization.

Practical large RISs can usually employ quantized phase shift as they are more cost-effective \cite{WZ20}. A two-stage approach to address the discrete phase shifts constraints is to project the continuous solution to the closest value in the discrete set \cite{WZ20,YBA20},\cite{YZZ20,ZSRLCL22}. Although, as shown in the present paper, the quantization approach can potentially provide high performance and low computational complexity, it can only give marginal insight on the actual optimum discrete phase shifts selection problem.

When it comes to designing algorithms with discrete phase shift constraints, as the number of possible solutions increases exponentially with the number of RIS elements, exponential search techniques are required \cite{XDMWQ22}, and a closed form solution is practically unavailable, as we discuss in Section \ref{sec:upqSec}. As an example, in \cite{XDMWQ22}, the authors stated that the discrete beamforming problem for RIS turns out to be a generally NP-hard discrete quadratic program. To achieve the optimal solution, most of the prior work in single-user scenarios had exponential complexity, sometimes over the number of RIS elements ($N$) \cite{WGWM23,WZ20}, and sometimes over the phase shift levels ($K$) \cite{JSDH21}.

To the best of our knowledge, there is still a gap in the literature for further research in the optimal discrete beamforming problem. Regarding the previously published work addressing the optimal discrete beamforming, the authors in \cite{SBRFZT21} pointed out that an $N$-step search algorithm for $K$-ary beamforming can be developed. In \cite{ZSRLCL22}, the authors provided a linear time optimal algorithm for the binary case, where $2N+2$ steps are required for convergence. Also in \cite{ZSRLCL22}, the authors provided an approximation algorithm (APX), and a simple quantization algorithm for $K$-ary beamforming, where the performance is evaluated over the estimated channels. Recently, the authors in \cite{9961233} proposed a $K$-ary optimal discrete beamforming algorithm with a polynomial search complexity, i.e., $2N(K-1)$ steps to ensure optimality. The authors in \cite{b1} proposed the first $K$-ary linear time algorithm with $KN$ steps to converge, which could be reduced to $2N$ steps when the direct link is not completely blocked.

In this work, we address the problem of optimizing discrete phases in an RIS to maximize the received power at a user equipment (UE) for a single-input single-output (SISO) system with full channel state information (CSI). The main contributions are given as follows:
\begin{itemize}
	\item We provide necessary and sufficient conditions to achieve this maximization. We employ these conditions to develop a linear time algorithm achieving provable optimality convergence in $N$ or \textit{fewer} steps, whether the direct link between the BS and the UE is blocked or not. Employing the geometric approach in \cite{b1}, we develop a formal elementwise update rule to be used, so that in each of those $N$ or \textit{fewer} steps, one or a small number of elements are updated, respectively.
	\item  We prove the periodicity in elementwise updates for the optimal beamforming, and exploit this periodicity to both reduce the number of steps, and to provide a simple initialization for the search algorithms. With this, we show the relation between the channel phases and the pattern of elements in which the periodicity must occur. 
	\item Our developed algorithms are shown to give a substantial reduction of computation time, as compared to the algorithms in the literature \cite{b1,ZSRLCL22,SBRFZT21,XDMWQ22}. Besides providing improved optimal discrete phase shift selection algorithms, this work gives further insights on the discrete beamforming optimization, with the periodicity rule.
	\item  We formally define an intuitive, quantization-based, discrete phase shift selection algorithm, which we will call uniform polar quantization (UPQ). We show that provided full CSI is available, it performs well, in terms of both performance and the computational time complexity. With UPQ, we reveal that the optimal discrete beamforming can be closely approximated as a quantization solution.
\end{itemize}
The received power maximization problem in this work is connected to generic $K$-ary discrete quadratic programming (QP), where the objective is to maximize $\mathbf{x}^{\mathrm{T}}\mathbf{Q}\mathbf{x}$, with $\mathrm{rank}(\mathbf{Q}) = 1$ \cite{b1,XDMWQ22}, where the single eigenvector is positive. Therefore, the linear time algorithms with the elemental update rules in the present paper can be employed in similar maximization problems, so that the global optimum can be achieved in linear time.

\begin{comment}
To the best of our knowledge, there is still a notable gap in the literature for developing low-complexity algorithms for achieving optimal received power with discrete phase shifts.

In this paper, we consider a single-antenna BS and a single-antenna UE, i.e. single-user single-input single-output (SU-SISO) system, where the BS-UE direct link suffers blockage. The reason for us to work on this simple scenario is to get more tractable and insightful results, similar to \cite{WZ19}, for our proposed algorithms.

%%% FROM b1 Linear Time Paper
The main purpose is to boost the signal reception at the target receiver.
The existing studies in this area [1b1] mainly divided into two categories: those assuming continuous phase shifts to ease optimization or analysis, and those restricting the phse shifts to a given discrete set rom a practical standpoint.

The algorithm stems from a geometric interpretation of the RIS beamforming problem which was first proposed in [3]. 

The existing works seldom consider global optimum for the discrete IRS beamforming. Although the IRS technology has been extensively studied over the past few years for many complicated system models, the simplest point-to-point model is still far less well understood.

A common practice in the literature is to first solve the relaxed continuous beamforming problem via standard optimization, and then round the solution to the discrete set, e.g., [4][5]

[12schober] resort to the branch-and-bound algorithm to ontain the global optimum of the discrete RIS beamforming. These methods incur exponential time complexities and provide limited insights.

with [10], The best result so far in the literature for K-ARY beamforming is to attain an approximation ratio of the global optimum, where [10] gives an approximation ratio of cos.. 

This work gives the first polynomial time algorithm for the discrete IRS beamforming with provable global optimality.

%%%OPTIMAL LOW COMPLEXITY PAPER
However, there is the need for discrete phase shift analysis to create the connection between the ideal and the practical realizations of RISs.

Most of the prior work on discrete phase shift beamforming in single-user scenario has shown optimal solutions to obtained with exponential complexity [7],[8]. 

As the number of possible combinations of discrete phase shifts grows exponentially with the number of elements.

%%% Aug22 Optimal Paper
in the existing literature [26],[32],[45],[46], a common way of discrete beamforming is to round the relaced xontinuous solution to the closest point in the discrete set. Referred to as CPP. This is shown that it can result in arbitrarily bad performance.

%%% INNER PRODUCT PAPER.
PG3: Mathematically, the phase configuration otpimization of riss in practical beamformign is subject to two constraints....

PG4: Accommodating the second discrete configuration constraint mentioned in PG3, the most straightforward approach is to round the continuous phase configuration on the nearest point in the discrete constraint set [39]-[42]. However, these two-stage approaches can lead to significant performance degradation [26USE THIS QWU], particularly when applied to extremely low-bit phase configurations. In the worst-case scenario, they may even result in arbitrarily poor performance [43aug22].

PG5:To comprehensively and optimally address the discrete challenge, a paradigm shift is required, involving the development of optimization approaches that directly handle the discrete phase configurations. However, it's essential to recognize that discrete optimization problems tend to fall within the universal (NP-hard) category, requiring resource-intensive exponential search techniques. In response to this challenge, researhers have put forward varuous techniques aimed at accelerating the search process, which include the successive refinement algorithm[26], the angle-of-arrival estimation similarity method [44] and the bnb algorithms, [4][45]. Moreover, an aproach based on training sets is introduced in [46],. The authors in [43] present an approximation (APX) algorithm to approximate the global optimal solution.

It should be noted that htese algorithms often converge to local optima. Tot he best of out knowledge, there exists a notable research gap regarding the development of highly efficient search algorithms capable of guaranteeing global optimality for discrete phase configurations. In this paper, we bridge this gap by redefining the power enhancement problems as discrete inner product maximizations. B leveraging the inherent structure of such problems, we introduce a mathematically equivalent formulation that dramatically reduces the search space.
\end{comment}




